On the Interaction of Relational Database Access Technologies in Open Source Java Projects

This article presents an empirical study of how the use of relational database access technologies in open source Java projects evolves over time. Our observations may be useful to project managers to make more informed decisions on which technologies to introduce into an existing project and when. We selected 2,457 Java projects on GitHub using the low-level JDBC technology and higher-level object relational mappings such as Hibernate XML configuration files and JPA annotations. At a coarse-grained level, we analysed the probability of introducing such technologies over time, as well as the likelihood that multiple technologies co-occur within the same project. At a fine-grained level, we analysed to which extent these different technologies are used within the same set of project files. We also explored how the introduction of a new database technology in a Java project impacts the use of existing ones. We observed that, contrary to what could have been expected, object-relational mapping technologies do not tend to replace existing ones but rather complement them.

==> coarse-grained.tex <==
%!TEX root=saner2016-longpaper.tex

\section{Coarse-grained study\label{sec:coarse-grained}}

For the coarse-grained analysis of Java database technologies,
we studied the evolution of technology usage at project level. 

Understanding when database technologies are first used and when they tend to be replaced or removed can help project managers to choose the most appropriate one. Trends in the moment of introduction of a particular technology can help identifying if the technology can be easily deployed in an existing projects, if it becomes more and more popular, etc. 
\tom{The above high-level paragraph can be useful as part of the abstract, introduction and/or conclusion as well.}

Introducing a new technology in a software project comes with a certain cost. A common policy is therefore to introduce such a technology only if the expected benefits outweigh the expected cost. Examples of such benefits are more efficient services, increased modularity, a reduced implementation or maintainance effort, etc.

Since database technologies are typically central components of the selected projects, we expect that these technologies are introduced very early in the projects' lifetimes. However, if most uses of a technology appear late in the projects' lifetimes, this may either indicate that is a quite recent technology or that the technology is well-suited to be introduced in existing projects.
\tom{I am not sure if the above paragraph should already be put here. It could be moved later, as part of a discussion, after presenting the obtained results...}

\subsection{How long does it take to make use of a technology?}

For each project, we analysed at what moment in the projects' lifetime each occurring database technology got introduced. 
We observed that the answer was strongly related to the duration of the considered projects. 
To take into account the effect of project duration, we normalized the lifetime of each project into a range of values between 0 (the start of the project) and 1 (the last considered commit).

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/starttimes.pdf}
    \caption{Violin plot (using a kernel density estimate) of the distribution of the introduction time of a technology.\label{fig:starttimes}}
\end{figure}

Figure~\ref{fig:starttimes} compares the distributions of the introduction time of a technology in a project. For each technology, we distinguish whether the technology is the first one that is introduced in a project or not. 

As expected, we observe that \textbf{more than 50\% of the introductions of a first database technology are done very early} (in the first 10\%) in the project's lifetime. For additional technologies introduced on top of an existing one, the distribution tends to be flatter.
%
Interestingly, we also observe that the two distributions for \jdbc present less differences than the ones related to \jpa or \hbm. This may indicate that \textbf{jdbc is less sensible to the order in which technologies are introduced}. 


\subsection{How long does it take to replace or complement an existing technology?}

To respond to this question, we use the statistical technique of \emph{survival analysis} to estimate the probability that a technology does not remain the last introduced one in a project lifetime. 
%
Survival analysis \cite{Samoladas2010} creates a model estimating the survival rate of a population over time, considering the fact that some elements of the population may leave the study, and for some other elements the event of interest does not occur during the observation period.
In our case, the observed event is the introduction in a project of another technology after an existing one.  

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{figures/survival_introduction_after.pdf}
\caption{Probability that a technology remains the last introduced technology over time.\label{fig:last_introduced}}
\end{figure} 

Figure~\ref{fig:last_introduced} shows the survival rates for each considered technology. 
%
We observe that \hbm has a much lower survival rate (\ie a lower probability of staying the last introduced technology for a long time) than the other technologies.
\textbf{Most projects tend to complement or replace \hbm more often than \jdbc or \jpa}. 
We also observe that, during the first 10\% of the projects' lifetime, the survival rates
of \hbm decrease by 30\%, representing a more important decrease than for the other two technologies. This implies that \textbf{\hbm is usually quickly replaced or complemented by another technology}.




==> fine-grained.tex <==
%!TEX root=saner2016-longpaper.tex

\section{Fine-grained study\label{sec:fine-grained}}

We explored so far the presence of \jdbc, \hbm or \jpa at project level. 
We saw in Table~\ref{tab:nb_by_techs} that many Java projects make use of several database technologies. 
%
As many projects use multiple technologies, either simultaneously or one after the other, it is useful to study how the introduction of a new technology can affect the presence of a previous one. Which combinations of technologies frequently co-occur in the selected Java projects? Such information would reveal which technologies are complementary, and which technologies are used as supporting technologies of other ones.

For technologies that tend to be replaced or complemented by other ones, can we determine when it occurs, and how long does it take? 
Does a new database technology appear in the same files than an existing one?

In order to answer these questions, we analyzed the files that are relate to the database technologies. The relations between source code files and database entities have been established as explained in Section~\ref{sec:methodo}.

\subsection{Does the introduction of a technology affect the presence of an existing one?}

The introduction of a new technology in a project could have an impact on the use of already included technologies. This impact, if it occurs, could result in an increase or a decrease of the usage of the existing technologies.

We identified and counted for which projects the introduction of a new technology has a positive impact (an increased use of the older technology), a negative impact (a decreased use of the older one) or no impact. 

\mg{I previously reformulated the above paragraph, since the word 'positive' could be misinterpreted: a more important use is not necessarly a good or bad thing. Should we reformulate?}

To qualify the impact, we used the first derivative of the number of files related to an existing technology. We computed the mean of this derivative for two 8-week time periods: a first period that ends when the new technology is introduced, and a second period that starts when the new technology is introduced. 

In the following, we will use the term {\em variation} to denote the difference between the mean of the second period and the mean of the first period. 

This variation gives an good idea of the trend: a positive value indicates an increasing use of the technology while a negative value indicates a decreasing use of the technology

Figure~\ref{fig:impact_value} shows the distribution of the variation for each pair of technologies. While \textbf{\jdbc and \hbm seem to have a positive impact on existing technologies}, this impact is much more important when introducing \hbm in a project that already uses \jpa. The converse is not true however: \textbf{introducing \jpa in a project that already makes use of \hbm seems to imply a decrease in the usage of \hbm}. 

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{figures/impact_value.pdf}
\caption{Impact of the introduction of a new technology on the activity of an other activity.\label{fig:impact_value}}
\end{figure}


\begin{figure*}[!htbp]
\centering
\includegraphics[width=1.5\columnwidth]{figures/impact_behavior_number.pdf}
\caption{Number of projects with an increasing, decreasing or stable technology activity when introducing another technology.\label{fig:impact_number}}
\end{figure*} 

Figure~\ref{fig:impact_value} only allowed to identify trends in our corpus of projects, it does not allowed to identify trends about the projects themselves. 
%
Figure~\ref{fig:impact_number} therefore shows the number of projects for which the existing technology has an increasing usage (red curve), decreasing usage (blue curve) or a stable usage (green curve) for several time values after the introduction of another technology. We can see that for most pairs of technologies, the number of projects having an increased or stable activity (of the technology that was already present) is greater than the number of those having a decreasing activity. Our analyses therefore seem to indicate that \textbf{most usages of existing technologies are not negatively affected by the introduction of another one}.
A notable exception are those projects where \jpa is being introduced after \hbm.





\subsection{How long does it take for a technology to be (partially) replaced by another one?}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=2\columnwidth]{figures/survival_remaining_files.pdf}
\caption{Probability that at least 25\% of files of a technology remains after the introduction of another technology.\label{fig:impact_remaining}}
\end{figure*}



Figure~\ref{fig:impact_remaining} shows survival curves, using a Kaplan-Meier estimator, of the probability that a project keeps more than (an arbitrary threshold of) $25\%$ of its files related to an existing technology after the introduction of another one.
\tom{Why 25\%? Appears to be an arbitrary value...}
\ad{Indeed. And I have no relevant explanation for this. We could probably explain that looking for $100\%$ is too strict, because even for projects in which we know a technology is no longer used, files related to this technology are still detected (but not used).}
This analysis confirms our previous observations: \textbf{the introduction of \jdbc does not seem to have a great impact on the usage of existing technologies, and neither does the introduction of \jpa or \hbm on an existing usage of \jdbc}. 
Again, we see that \textbf{the most important behaviors are exhibited by \jpa and \hbm}: the probability to keep more than $25\%$ of files related to \hbm drops below $0.55$ when introducing \jpa while this probability drops to a little more than $0.6$ when introducing \hbm after \jpa.

Notice from Figures~\ref{fig:impact_number} and~\ref{fig:impact_remaining} that \textbf{most of the observed impacts occur in the very first weeks after the introduction of a new technology}. 
\ad{We should keep this last sentence only if we do something with it, like trying to justify why we focus on the very first weeks in the following RQ's.}


\tom{CONTINUE PROCESSING FROM HERE...}

\subsection{How are technologies spread over files?}

We observed that the use of \jdbc is not really impacted by the use of \jpa or \hbm. 
Contrarily, we observed that the use of \jpa (resp. \hbm) is influenced by the use of \hbm (resp. \jpa), suggesting that \jpa and \hbm replace one another more than they complement each other. 

We therefore studied the presence of those technologies in each file of each project, in order to see if this complementarity can also be observed at file level.
In particular, we are interested to identify which are the pairs of technologies that tend to be used in the same set of files, and which are the pairs of technologies that tend to be used in disjoint subsets of files. 

\ad{Continue process from here}

Figure~\ref{techno-relative-purity} shows, for each pair of technologies, the distribution of the relative number of files in which only one technology, or both technologies, have been introduced in their entire lifetime, per project. For a considered pair of technologies, only projects in which both technologies have been introduced have been retained as element of the distribution.

\begin{figure*}[tbp]
	\centering
	    \begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/technology-purity-hbm-jdbc}
	        \caption{Hibernate and JDBC\label{techno-relative-purity-hbm-jdbc}}
	    \end{subfigure}%
	    ~ 
		\begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/technology-purity-jdbc-jpa}
	        \caption{JDBC and JPA\label{techno-relative-purity-jdbc-jpa}}
	    \end{subfigure}
		~
	    \begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/technology-purity-hbm-jpa}
	        \caption{Hibernate and JPA\label{techno-relative-purity-hbm-jpa}}
	    \end{subfigure}
	\caption{Distribution of the relative number of files having one of the considered of technologies, or both of them.\label{techno-relative-purity}}
\end{figure*}
 
Figures~\ref{techno-relative-purity-hbm-jdbc} and \ref{techno-relative-purity-jdbc-jpa} reveals that pairs of technologies including JDBC present similar profiles: Most projects contain a small number of files using both technologies. A Mann-Whitney U test confirms this similarity between distributions: the null hypothesis that states that the distributions associated to the number of files using a single technology are identical can not be rejected ($p = 0.071$ and $0.287$, respectively). We conclude that \textbf{\jdbc is generally not used in the same files that JPA and Hibernate}.

\jpa and \hbm form a pair of technologies presenting a different behaviour. The distributions of the number of files that only relate to these technologies are significantly different ($p < 0.001$): \textbf{while \jpa is generally used alone, \hbm-related files also contains \jpa annotations}. The number of files that use both technologies is also more important for \hbm and \jpa than the other considered pairs of technologies.

To summarize, there is a clear separation between files using \jdbc and files using the two other technologies. For \hbm and \jpa, a partial, asymetric overlap exists: at file level, \hbm is often used in the same files than \jpa, while \jpa is mostly used alone.


\subsection{Are there technology migrations?}

In the previous section, we observed that \hbm and \jpa may be found in the same files. In order to determine if these technologies are used simultaneously, or if a technology migration can be observed over time, we analyzed how the files that related to a technology are changed when a second technology is introduced in their associated projects. 

For each project in which a technology $A$ has been introduced before a technology $B$, we define the \emph{initial files} as the set of files that were belonging to the project and that were related to $A$ when $B$ has been introduced in the project. At any time $t$ after the introduction of $B$, a \emph{profile} is associated to the project, depending on the status of the majority of its initial files at that time.
\begin{itemize}
	\item A project is considered as \textbf{residual} if a majority of its initial files still relate to $A$ and not to $B$.
	\item A \textbf{suppression} project is a project in which most initial files do no longer relate to $A$, nor $B$.
	\item \textbf{Completion} projects are project in which a majority of inital files simultaneously relate to $A$ and $B$.
	\item Projects in which most initial files do no longer relate to $A$ and relate to $B$ are considered as \textbf{replacement} projects.	
\end{itemize} 

Figure~\ref{fig:existing-file-contamination} shows the evolution of the relative number of projects belonging to each profile over time.

\begin{figure*}[htbp]
	\centering
	    \begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/migration-trend-evolution-JDBC-JPA}
	        \caption{JPA after JDBC}
	    \end{subfigure}%
	    ~ 
	    \begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/migration-trend-evolution-JPA-JDBC}
	        \caption{JDBC after JPA}
	    \end{subfigure}
	    ~
		\begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/migration-trend-evolution-Hibernate-JDBC}
	        \caption{JDBC after Hibernate}
	    \end{subfigure}\\
		
		\begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/migration-trend-evolution-JDBC-Hibernate}
	        \caption{Hibernate after JDBC}
	    \end{subfigure}
		~
		\begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/migration-trend-evolution-JPA-Hibernate}
	        \caption{Hibernate after JPA}
	    \end{subfigure}
		~
		\begin{subfigure}[t]{0.3\textwidth}
	        \centering
	        \includegraphics[width=\textwidth]{figures/migration-trend-evolution-Hibernate-JPA}
	        \caption{JPA after Hibernate}
	    \end{subfigure}
		
	\caption{Evolution of the relative number of projects belonging to each profile.\label{fig:existing-file-contamination}}
\end{figure*}

For transitions in which \jdbc is the first technology, replacement and completion are the dominant profiles in less than 3\% of all projects. That reveals a very low impact of the introduction of \jdbc and \hbm on initial files. The projects mostly belong to the \emph{residual} profile during the entire observation period, even if, over time, an increasing number of projects leave this profile for adopting the \emph{suppression} profile. 

A similar behaviour is observed for projects in which \jdbc is the lately introduced technology: at most 4.5\% of projects have a majority of inital files being adapted to \jdbc, and the vast majority of projects tend to not predominantly modify their files in order to benefit from the introduction of \jdbc in the project.

The same lack of adaptation of the inital files is observed when \hbm is introduced after \jpa. One month after the introduction of the second technology, 75\% of the concerned projects are still associated to the \emph{residual} profile. For this transition, completions and replacements are clearly observed in few projects, but this adoption is only a short-term behaviour: one month after the introduction of \hbm, no projects remain associated to the \emph{completion} or the \emph{replacement} profiles. While most projects are associated to the \emph{residual} profile during the entire observation period, the number of projects in which most of initial \jpa-related files loss their relation to \jpa constently increases over time. Consequently, the single long-term project behaviour we observed consists in not introducing \hbm in the initial \jpa-related files, until \jpa is removed from most of these files.

The transition from \hbm to \jpa presents more diversified project profiles. As is the case for the other transitions, \emph{residual} is the most often adopted profile, which means that most \hbm-related files are not modified to benefit from \jpa annotations. A evolutionary suppression pattern similar to that which has been observed in the other transitions can be seen when \jpa is introduced: the relative number of projects that suppressed a majority of the initially existing \hbm-related files increases over time to reach 26\% 14 weeks after the introduction of \jpa. Contrary to the other transitions, a clear completion or replacement behaviour can be observed in 3.6\% and 14.3\% of the considered projects (respectively). This predominant adaptation of the initial files can be observed as soon as the \jpa technology is introduced in the concerned projects, and the number of projects in which \jpa has been used to complete or to replace \hbm in initial files is relativelly stable over time. The relative importance of the \emph{replacement} profile could bring to light the determination of some project developpers to use \jpa as an alternative to \hbm, even for files in which \hbm is already present and supposedly used. 

To sum up, whatever the considered transition, \textbf{the most commonly adopted behaviour consists in not modifying the files that initially relate to the first technology} in order to benefit from the lately introduced one. Over time, an increasing number of projects tend to remove the first considered technology from a majority of the files in which the technology was initialy present.\textbf{ This removal is not part of a project migration} from the first technology to the lately one, since the second technology is not introduced in the same proportion in the concerned files. The introduction of \jpa after \hbm is the only transition in which a significant long-term migration has been observed.  

I suggest to simply trow these subsections away, since they provide useless views of the distribution of initial files. 

% \subsection{*}
% A file distribution, over projects. In the distribution, each value is the relative number of files having a technology A when a technology B has been introduced, that also finish by having B.
% 
% \begin{figure}[tbp]
% \centering
% \includegraphics[width=\columnwidth]{figures/contamination-ratio.pdf}
% \caption{Relative number of files being t1-related that also finished by being t2-related. Distribution over projects}
% \end{figure}
% 
% Things seem logical here: The only situations where we observe a significant file contamination ration is from Hibernate to JPA, and, with lower values, JPA to Hibernate. The other combinations are too rare to be significant. Despite the fact we observe a simple dashed line for the other boxplots, there are different values associated to these groups, but pandas does not represent them. 
% 
% 
% 
% \subsection{*}
% 
% Relative number of files having A when B was introduced in the project, and that have B not later than 15 weeks after B has been introduced in the project. This figure is quite similar to the previous one (which is normal, because most of the changes occur before 15 weeks). To summarize, JDBC files are not contaminated by JPA and Hibernate, and JPA and Hibernate are not contaminated by JDBC. There are some transitions from and to Hibernate and JPA (mostly, from Hibernate to JPA): when JPA is introduced, it tends to take the place Hibernate has taken before; while Hibernate is introduced, it does not tend to take the same files JPA taken before. So JPA is probably a substitute to Hibernate, while Hibernate is introduced in projects (where JPA is already present) to offer an additional support to new files and to complement JPA.
% 
% \begin{figure}[tbp]
% \centering
% \includegraphics[width=\columnwidth]{figures/contamination-ratio-15w.pdf}
% \caption{Relative number of files being t1-related that also finished by being t2-related after 15 weeks. Distribution over projects.}
% \end{figure}
% 
% \subsection{*}
% 
% For each week that follows the introduction of JPA/Hibernate, the proportion of Hibernate/JPA files that have been contaminated by the introduced technology. This is not a cumulative view. The third figure shows the evolution of contamination from any technology to any other technology.
% \begin{figure}[tbp]
% \centering
% \includegraphics[width=\columnwidth]{figures/contamination-jpa-hbm-evol.pdf}
% \caption{Relative number of files being JPA-related that become Hibernate-related during the considered week. Distribution over projects.}
% \end{figure}
% 
% \begin{figure}[tbp]
% \centering
% \includegraphics[width=\columnwidth]{figures/contamination-jpa-hbm-evol.pdf}
% \caption{Relative number of files being Hibernate-related that become JPA-related during the considered week. Distribution over projects.}
% \end{figure}
% 
% \begin{figure}[tbp]
% \centering
% \includegraphics[width=\columnwidth]{figures/contamination-global-evol.pdf}
% \caption{Relative number of files being t1-related that become t2-related during the considered week, for any distinct t1 and t2. Distribution over projects.}
% \end{figure}
% 
% In both case, most of the contamination occurs during week 0, and I cannot see anything interesting for the other weeks.

==> future.tex <==
%!TEX root=saner2016-longpaper.tex

%\section{Future Work}
%\label{sec:future}

The research presented in this paper can be extended in many ways.

\ad{Ideas:}
\begin{itemize}
  \item Extend to more Java projects, on github or elsewhere.
  \item Include other database-mapping technologies.
  \item Do not only consider relational databases (eg. NoSQL, Redis, ...)
  \item Use a finer granularity that file level (like LoC level?)
  \item Correlate our results with well-known metrics (incl. \#bugs!)
\end{itemize}
%


==> related.tex <==
%!TEX root=saner2016-longpaper.tex

\section{Related Work}
\label{sec:related}

In \cite{GoeminnetEtAl2014}, we empirically analysed the evolution of the usage of SQL, Hibernate and JPA in a single large open source Java project. The current paper builds further upon that research by carrying out a macro-level study on thousands of projects.
%
Chen et al.~\cite{ChenSJHNF2014} proposed a static code analysis framework for detecting and fixing performance issues and potential bugs in ORM usage. Their analysis revealed that the modifications made after analysis caused an important improvement of the studied systems' response time.
 %
Maule et al.~\cite{Maule2008} studied a commercial object-oriented content management system to statically analyse the impact of  database schema changes on the source code. Qiu et al.~\cite{Qiu2013-FSE-DB} empirical analysed the co-evolution of database schemas and code in ten open-source database applications from various domains. Whereas our  focus is on Java projects, they studied specific change types inside the database schema and the impact of such changes on PHP code.

The statistical technique of \emph{survival analysis} used in this paper has been employed by other software engineering researchers as well.
Samoladas \etal \cite{Samoladas2010} predicted the survivability of open source projects over time.
Scanniello \cite{Scanniello2011} analysed dead code in five open source Java software systems.
Kyriakakis \etal \cite{Kyriakakis2014} studied function usage and function removal in five large PHP applications.
Claes \etal \cite{Claes2015MSR} studied the survival of installability conflicts in Debian packages.

